Efficient Privacy-Preserving Electricity Theft Detection with Dynamic Billing and Load Monitoring for AMI Networks

In advanced metering infrastructure (AMI), smart meters (SMs) are installed at the consumer side to send fine-grained power consumption readings periodically to the system operator (SO) for load monitoring, energy management, billing, etc. However, fraudulent consumers launch electricity theft cyber-attacks by reporting false readings to reduce their bills illegally. These attacks do not only cause financial losses but may also degrade the grid performance because the readings are used for grid management. To identify these attackers, the existing schemes employ machine-learning models using the consumers' fine-grained readings, which violates the consumers' privacy by revealing their lifestyle. In this paper, we propose an efficient scheme that enables the SO to detect electricity theft, compute bills, and monitor load while preserving the consumers' privacy. The idea is that SMs encrypt their readings using functional encryption, and the SO uses the ciphertexts to (i) compute the bills following dynamic pricing approach, (ii) monitor the grid load, and (iii) evaluate a machine-learning model to detect fraudulent consumers, without being able to learn the individual readings to preserve consumers' privacy. We adapted a functional encryption scheme so that the encrypted readings are aggregated for billing and load monitoring and only the aggregated value is revealed to the SO. Also, we exploited the inner-product operations on encrypted readings to evaluate a machine-learning model to detect fraudulent consumers. Real dataset is used to evaluate our scheme, and our evaluations indicate that our scheme is secure and can detect fraudulent consumers accurately with low communication and computation overhead.

==> Files/bio.tex <==
\section*{Biographies}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/Mohamed_Ibrahem.png}}]{Mohamed I. Ibrahem}
	is currently a Graduate Research Assistant in the Department of Electrical \& Computer Engineering, Tennessee Tech. University, USA and pursuing his Ph.D. degree in the same department.
	He received the B.S. degree and the M.S. degree in Electrical Engineering (electronics and communications) from Benha University, Cairo, Egypt in 2014 and 2018, respectively.
	His research interests include machine learning, cryptography and network security, and privacy preserving schemes for smart grid communication and AMI networks.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/mahmoud_nabil.jpg}}]{Dr. Mahmoud Nabil}
	is currently an Assistant Professor in the Department of Electrical and Computer Engineering, North Carolina A \& T University.
	He received the B.S. degree and the M.S. degree in Computer Engineering from Cairo University, Cairo, Egypt in 2012 and 2016, respectively, and the Ph.D. degree from Tennessee Technological University, TN, USA in 2019.
	His research interests include machine learning, cryptography and network security, smart-grid and AMI networks, and vehicular ad-hoc networks.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/mfouda.jpg}}]{Dr. Mostafa M. Fouda} (SM'14) is currently an associate professor at Benha University (Egypt), and an adjunct graduate faculty member at Tennessee Technological University (USA). He is also a former assistant professor at Tohoku University (Japan). Dr. Fouda received his B.S. (with Hons.) and M.S. degrees from Benha University (Egypt) in 2002 and 2007, respectively, and his Ph.D. degree from Tohoku University (Japan) in 2011. He has published over 30 papers mostly in IEEE conference proceedings and journals. His research has been cited more than 1200 times. He has served on the technical committees of several IEEE conferences such as IEEE ICC, GLOBECOM, etc. He is also a reviewer in several IEEE Transactions/Magazines and an associate editor of IEEE Access.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/mohamed_mahmoud.jpg}}]{Dr. Mohamed M. E. A. Mahmoud}
	received PhD degree from the University of Waterloo in April 2011. From May 2011 to May 2012, he worked as a postdoctoral fellow in the Broadband Communications Research group - University of Waterloo. From August 2012 to July 2013, he worked as a visiting scholar in University of Waterloo, and a postdoctoral fellow in Ryerson University. Currently, Dr. Mahmoud is an associate professor in Department Electrical and Computer Engineering, Tennessee Tech University, USA. The research interests of Dr. Mahmoud include security and privacy preserving schemes for smart grid communication network, mobile ad hoc network, sensor network, and delay-tolerant network. Dr. Mahmoud has received NSERC-PDF award. He won the Best Paper Award from IEEE International Conference on Communications (ICC'09), Dresden, Germany, 2009. Dr. Mahmoud is the author for more than twenty three papers published in major IEEE conferences and journals, such as INFOCOM conference and IEEE Transactions on Vehicular Technology, Mobile Computing, and Parallel and Distributed Systems. He serves as an Associate Editor in Springer journal of peer-to-peer networking and applications. He served as a technical program committee member for several IEEE conferences and as a reviewer for several journals and conferences such as IEEE Transactions on Vehicular Technology, IEEE Transactions on Parallel and Distributed Systems, and the journal of Peer-to-Peer Networking.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/Waleed.jpg}}]{Dr. Waleed Alasmary}(SM'19) received the B.Sc. degree (Hons.) in computer engineering from Umm Al-Qura University, Saudi Arabia, in 2005, the M.A.Sc. degree in electrical and computer engineering from the University of Waterloo, Canada, in 2010, and the Ph.D. degree in electrical and computer engineering from the University of Toronto, Toronto, Canada, in 2015. During his Ph.D. degree, he was a Visiting Research Scholar with Network Research Laboratory, UCLA, in 2014. He was a Fulbright Visiting Scholar with CSAIL Laboratory, MIT, from 2016 to 2017. He subsequently joined the College of Computer and Information Systems, Umm Al-Qura University, as an Assistant Professor of computer engineering. His ``Mobility impact on the IEEE 802.11p'' article is among the most cited Ad Hoc Networks journal articles list from 2016-2018. He published articles in prestigious conferences and journals, such as the IEEE Transactions on Vehicular Technology and the IEEE Communications Surveys and Tutorials. His current research interests include mobile computing, ubiquitous sensing, and intelligent transportation systems, privacy and anonymity.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Files/Pics/Fawaz.jpg}}]{Dr. Fawaz Alsolami}
received the M.A.Sc in Electrical and Computer Engineering from
University of Waterloo, Canada, in 2008, and his Ph.D. degree in Computer Science from KAUST University, Thuwal, Saudi Arabia, in 2016. Fawaz joined computer science at King Abdulaziz University as an assistant professor of Computer Science. His research interests are artificial Intelligence, machine learning and data Mining, and combinatorial optimization. He also published many articles and one monograph. He has been the chairman of the Computer Science department at King Abdulaziz University since 2018.
\end{IEEEbiography}
